Hierarchically Integrated Models: Learning to Navigate from Heterogeneous Robots

Deep reinforcement learning algorithms require large and diverse datasets in order to learn successful policies for perception-based mobile navigation. However, gathering such datasets with a single robot can be prohibitively expensive. Collecting data with multiple different robotic platforms with possibly different dynamics is a more scalable approach to large-scale data collection. But how can deep reinforcement learning algorithms leverage such heterogeneous datasets? In this work, we propose a deep reinforcement learning algorithm with hierarchically integrated models (HInt). At training time, HInt learns separate perception and dynamics models, and at test time, HInt integrates the two models in a hierarchical manner and plans actions with the integrated model. This method of planning with hierarchically integrated models allows the algorithm to train on datasets gathered by a variety of different platforms, while respecting the physical capabilities of the deployment robot at test time. Our mobile navigation experiments show that HInt outperforms conventional hierarchical policies and single-source approaches.

==> tikz/method_diagram.tex <==
% We need layers to draw the block diagram
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

% Define a few styles and constants
\tikzstyle{arrownode}  = [above, text width=5em]
\tikzstyle{emptynode}  = [text centered, minimum height=2.5em]
\tikzstyle{bluenode}   = [emptynode, draw, fill=blue!20, text width=2.5em]
\tikzstyle{photonode}   = [emptynode, draw, fill=black!20, text width=2.5em]
\tikzstyle{photonodehigh}   = [emptynode, draw, fill=black!20, text width=2.5em, text height=5em]
% \tikzstyle{rednode}    = [emptynode, draw, fill=red!25,  text width=2em]
\tikzstyle{rednode}    = [emptynode, draw, circle, fill=red!25, text width=1.5em]
\tikzstyle{bigrednode} = [emptynode, draw, fill=red!12,  text width=11em, text height=6em, rounded corners]
\tikzstyle{medrednode} = [emptynode, draw, fill=red!12,  text width=3.6em, text height=5em, rounded corners]
\tikzstyle{yellownode} = [emptynode, fill=\coloryellow, text width=.5em, text height=.3em, minimum height=.3em]

% \def\datum{$\bs_t,\!\ba_t,\!\bs_{t\!+\!1}$}
% \def\datum{$\bs,\!\ba,\!\bs'$}
\def\blockdist{1.94}
\def\shifttop{0.8}
\def\shiftmid{-0.1}
\def\shiftbot{-1}
\def\shifttikz{0mm}


\tikzstyle{dpernode} = [emptynode, draw, fill=red!12,  text width=8em, cylinder, shape border rotate=90, aspect=0.05]
\tikzstyle{ddynnode} = [emptynode, draw, fill=red!12,  text width=5em, cylinder, shape border rotate=90, aspect=0.1]
\tikzstyle{robotnode}   = [emptynode, draw, fill=blue!20, text width=3.8em]
\tikzstyle{trainpernode} = [emptynode, draw, fill=green!12,  text width=8em, rounded corners]
\tikzstyle{traindynnode} = [emptynode, draw, fill=green!12,  text width=5em, rounded corners]
\tikzstyle{plannernode} = [emptynode, draw, fill=cyan!12,  text width=8em, rounded corners]



\begin{figure}[!b]
\vspace*{-20pt}
\begin{minipage}{\columnwidth}
\begin{figure}[H]
{\footnotesize
\begin{tikzpicture}
    \hspace{\shifttikz}
    
    \node (dpernode) [dpernode] {$\datasetperception$};

    % ==========================================================
    % Training perception
    % ==========================================================

    %%%% Robots
    \def\robotshift{4.5em}
    % photos
    \path (dpernode)+(-2.0em,\robotshift) node (robot1) [photonode, fill zoom image*={clip,trim=0 0 0 14cm}figures/real/data_sources/kobuki.jpg]  {};
    \path (dpernode)+(0.5em,\robotshift)  node (robotdots)  [emptynode] {$\hdots$};
    \path (dpernode)+(+3.0em,\robotshift) node (robotK) [photonode, fill overzoom image=figures/real/data_sources/gopro.jpg]  {};
    % texts
    \def\robottextshift{1.7em}
    \path (robot1)+(0,\robottextshift) node (robot1text)    [emptynode]  {Robot 1};
    \path (robotK)+(0,\robottextshift) node (robotKtext)    [emptynode]  {Robot K};
    \path (robot1)+(0.5em,-2em) node (robot1datatext) [emptynode] {$(\bo, \bp, r)$};
    \path (robotK)+(0.5em,-2em) node (robotKdatatext) [emptynode] {$(\bo, \bp, r)$};
    % lines
    \draw[->] (robot1) -- node [right] {} (robot1.south west) -- (robot1.south west |- dpernode.north);
    \draw[->] (robotK) -- node [right] {} (robotK.south west) -- (robotK.south west |- dpernode.north);
    
	%%%% Training
    \def\trainingshift{3.5em}
	\path (dpernode)+(0em,-\trainingshift) node (trainpernode) [trainpernode] {Train $\fperception_\theta$};
    % lines
    \draw[->] (dpernode) -- node [right] {} (dpernode |- trainpernode.north);

    % ==========================================================
    % Training dynamics
    % ==========================================================
    
	\def\dynshift{9.5em}    
    
    %%%% dataset
    \path (dpernode)+(\dynshift,0) node (ddynnode) [ddynnode] {$\datasetdynamics$};
    
    %%%% robot
    \path (ddynnode)+(0,\robotshift) node (robotdynnode) [photonode, fill overzoom image=figures/real/data_sources/jackal.jpg]  {};
    \path (robotdynnode)+(0,\robottextshift) node (robotdyntextnode)    [emptynode]  {Robot};
    \path (robotdynnode)+(0.5em,-2em) node (robotdyndatatext) [emptynode] {$(\bs, \ba, \bp)$};
    \draw[->] (robotdynnode) -- node [right] {} (robotdynnode.south west) -- (robotdynnode.south west |- ddynnode.north);
    
    %%%% Training
    \path (ddynnode)+(0,-\trainingshift) node (traindynnode) [traindynnode] {Train $\fdynamics_\phi$};
    \draw[->] (ddynnode) -- node [right] {} (ddynnode |- traindynnode.north);
    
    % ==========================================================
    % Training
    % ==========================================================
    
    \path (robot1.north west)+(0.5,0.55) node (training) {\lightgrey{Perception}};
    \path (robotdynnode.north west)+(0.25,0.55) node (training) {\lightgrey{Dynamics}};
    \path (robot1.north west)+(0.0,0.95) node (training) {\lightgrey{Training}};

    % Now it's time to draw the colored data and training rectangles.
    % To draw them behind the blocks we use pgf layers. This way we  
    % can use the above block coordinates to place the backgrounds   
    \begin{pgfonlayer}{background}
        \hspace{\shifttikz}
        % training background
        \path (robot1.north west)+(-0.55,0.8) node (a) {}; % helper coordinate
        \path (traindynnode.south east)+(+0.3,-0.3) node (b) {};   % helper coordinate
        \path[fill=yellow!20,rounded corners, draw=\colorlightgrey, dashed] (a) rectangle (b);
        % training perception background
        \path (robot1.north west)+(-0.4,0.4) node (a) {}; % helper coordinate
        \path (trainpernode.south east)+(+0.38,-0.2) node (b) {}; % helper coordinate
        \path[fill=gray!10,rounded corners, draw=\colorlightgrey, dashed] (a) rectangle (b);
        % training dynamics background
        \path (robotdynnode.north west)+(-0.6,0.4) node (a) {}; % helper coordinate
        \path (traindynnode.south east)+(+0.2,-0.2) node (b) {}; % helper coordinate
        \path[fill=gray!10,rounded corners, draw=\colorlightgrey, dashed] (a) rectangle (b);
    \end{pgfonlayer}
    
    % ==========================================================
    % Deployment
    % ==========================================================
    
    % nodes
    \path (trainpernode)+(-1em,-6.0em) node (deployrobotnode)    [photonode, fill overzoom image=figures/real/data_sources/jackal.jpg]  {};
    \path (deployrobotnode)+(0,\robottextshift) node (deployrobottextnode)    [emptynode]  {Robot};    
    \path (deployrobotnode)+(9em,0) node (plannernode)    [plannernode]  {Plan using $\fcombo_{\theta,\phi}$};
    % lines
    \draw[->] (deployrobotnode) -- node [above] {$(\bo, \bs)$} (plannernode.west);
    \draw[->] (plannernode.south) |- +(0,-0.5em) node [right] {$\ba^*$} |- +(-2.8,-1.15em) -| (deployrobotnode.south); 
    
    \draw[->] (trainpernode.south) |- +(0,-1.5em) node [right] {$\theta$} |- +(0,-2.0em) |- +(3.,-2.0em) -|(plannernode.north); 
    \draw[->] (traindynnode.south) |- +(0,-1.5em) node [left] {$\phi$} |- +(0,-2.0em) |- +(-0.8,-2.0em) -|(plannernode.north); 

	% text
    \path (robot1.north west)+(0.3,-3.95) node (training) {\lightgrey{Deployment}};

    \begin{pgfonlayer}{background}
        \hspace{\shifttikz}
        % deployment background
        \path (robot1.north west)+(-0.55,-4.10) node (a) {}; % helper coordinate
        \path (traindynnode.south east)+(+0.3,-2.35) node (b) {};   % helper coordinate
        \path[fill=yellow!20,rounded corners, draw=\colorlightgrey, dashed] (a) rectangle (b);
    \end{pgfonlayer}

\end{tikzpicture}}
\end{figure}
\end{minipage}
\begin{minipage}{\columnwidth}
\caption{During training, we first gather perception data using a number of robots, such as indoor or outdoor ground vehicles, or even people walking around recording videos. For each of these robots, we save the onboard observations, change in poses, and rewards into a shared dataset, and use this dataset to train the perception model. Then, using the robot we will deploy at test time, we gather dynamics data by having the robot act in the real world and recording the robot's onboard states and actions into a dataset, and then use this dataset to train the dynamics model. When deploying, we combine the perception and dynamics model into a single integrated model. The robot then then plans a sequence of actions that maximizes reward, executes the first action, and repeats this planning process until the task is complete.}
\label{fig:method-diagram}
\end{minipage}
\end{figure}

